Assumption Generation for the Verification of Learning-Enabled Autonomous Systems

Providing safety guarantees for autonomous systems is difficult as these systems operate in complex environments that require the use of learning-enabled components, such as deep neural networks (DNNs) for visual perception. DNNs are hard to analyze due to their size (they can have thousands or millions of parameters), lack of formal specifications (DNNs are typically learnt from labeled data, in the absence of any formal requirements), and sensitivity to small changes in the environment. We present an assume-guarantee style compositional approach for the formal verification of system-level safety properties of such autonomous systems. Our insight is that we can analyze the system in the absence of the DNN perception components by automatically synthesizing assumptions on the DNN behaviour that guarantee the satisfaction of the required safety properties. The synthesized assumptions are the weakest in the sense that they characterize the output sequences of all the possible DNNs that, plugged into the autonomous system, guarantee the required safety properties. The assumptions can be leveraged as run-time monitors over a deployed DNN to guarantee the safety of the overall system; they can also be mined to extract local specifications for use during training and testing of DNNs. We illustrate our approach on a case study taken from the autonomous airplanes domain that uses a complex DNN for perception.

==> code/code_prism_full.tex <==
\begin{lstlisting}[language={Prism},
 breaklines=true, breakatwhitespace=true, 
firstnumber=1, firstline=1, 
caption={TaxiNet system (with lower accuracy DNN).},
label={prism_full_low}]
dtmc

const N;

module taxinet
	// State
    // cte=-1, he=-1: ERROR states
    // cte=1: center
    // cte=0: left margin
    // cte=2: right margin
    // he=1: negative angle
    // he=0: no angle
    // he=2: positive angle
	cte : [-1..2] init 1;
	he: [-1..2] init 0;
	
	// Estimate of the State from DNN
    cte_est: [0..2] init 0;
	he_est: [0..2] init 0; 
	

	// Actions Issued by Controller
    // a=0: go straight
    // a=1: turn left
    // a=2: turn right
    a: [0 .. 2] init 0; 

  	// Program Counter
	pc:[1..6] init 1; 

	// Steps
	k:[1..N] init 1;

    // Monitor State
	Q:[-1..6] init 0;

    // M2 = Sensor || Perception (Lower Accuracy)
	[] cte=1 & pc=1 -> 0.962: (cte_est'=1) & (pc'=2) + 0.002: (cte_est'=0) & (pc'=2) + 0.036: (cte_est'=2) & (pc'=2);
	[] cte=0  & pc=1 -> 0.681: (cte_est'=1) & (pc'=2) + 0.319: (cte_est'=0) & (pc'=2);
    [] cte=2 & pc=1 -> 0.398: (cte_est'=1) & (pc'=2) + 0.602: (cte_est'=2) & (pc'=2);

	[] he=0 & pc=2 -> 0.675: (he_est'=0) & (pc'=3) + 0.304: (he_est'=1) & (pc'=3) + 0.021: (he_est'=2) & (pc'=3); 	
	[] he=1 & pc=2 -> 0.043: (he_est'=0) & (pc'=3) + 0.957: (he_est'=1) & (pc'=3);
	[] he=2 & pc=2 -> 0.377: (he_est'=0) & (pc'=3) + 0.107: (he_est'=1) & (pc'=3) + 0.516: (he_est'=2) & (pc'=3);
	
	// Safety Monitor
	[] Q=0 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & he_est=0) | (cte_est=2 & he_est=1)) -> 1: (Q'=0) & (pc'=4);
	[] Q=0 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=1) & (pc'=4);
	[] Q=0 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=4) & (pc'=4);

	[] Q=1 & pc=3 & ((cte_est=0) | (cte_est=1 & he_est<2) | (cte_est=2 & he_est=1)) -> 1: (Q'=-1) & (pc'=6);
	[] Q=1 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=2) & (pc'=4);

	[] Q=2 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=-1) & (pc'=6);
	[] Q=2 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & he_est=0) | (cte_est=2& he_est=1)) -> 1: (Q'=2) & (pc'=4);
	[] Q=2 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=3) & (pc'=4);

	[] Q=3 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=-1) & (pc'=6);
	[] Q=3 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=0) & (pc'=4);
	[] Q=3 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & he_est=0) | (cte_est=2 & he_est=1)) -> 1: (Q'=4) & (pc'=4);

	[] Q=4 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & (he_est=0 | he_est=2)) | (cte_est=2)) -> 1: (Q'=-1) & (pc'=6);
	[] Q=4 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=5) & (pc'=4);

	[] Q=5 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=-1) & (pc'=6);
	[] Q=5 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & he_est=0) | (cte_est=2 & he_est=1)) -> 1: (Q'=5) & (pc'=4);
	[] Q=5 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=6) & (pc'=4);

	[] Q=6 & pc=3 & ((cte_est=0 & he_est<2) | (cte_est=1 & he_est=1)) -> 1: (Q'=-1) & (pc'=6);
	[] Q=6 & pc=3 & ((cte_est=1 & he_est=2) | (cte_est=2 & (he_est=0 | he_est=2))) -> 1: (Q'=0) & (pc'=4);
	[] Q=6 & pc=3 & ((cte_est=0 & he_est=2) | (cte_est=1 & he_est=0) | (cte_est=2 & he_est=1)) -> 1: (Q'=1) & (pc'=4);

    // Controller 
	[] cte_est=1 & he_est=0  & pc=4 -> 1: (a'=0) & (pc'=5);
	[] cte_est=1 & he_est=1 & pc=4 -> 1: (a'=2) & (pc'=5);
	[] cte_est=1 & he_est=2 & pc=4 -> 1: (a'=1) & (pc'=5);
	[] cte_est<1 & (he_est=0 | he_est=1) & pc=4 -> 1: (a'=2) & (pc'=5);
    [] cte_est<1 & he_est=2 & pc=4 -> 1: (a'=0) & (pc'=5);
    [] cte_est>1 & (he_est=0 | he_est=2) & pc=4 -> 1: (a'=1) & (pc'=5);
	[] cte_est>1 & he_est=1 & pc=4 -> 1: (a'=0) & (pc'=5);                                
	
	// Dynamics
	[] ((he=1 & a=1) | (he=2 & a=2)) & pc=5 & k<N -> 1: (he'=-1) & (pc'=6); // error
	[] ((cte=0 & he=0 & a=1) | (cte=2 & he=0 & a=2)) & pc=5 & k<N -> 1: (cte'=-1) & (pc'=6); // error
	[] ((cte=0 & he=1 & a=0) | (cte=2 & he=2 & a=0)) & pc=5 & k<N -> 1: (cte'=-1) & (pc'=6); // error
	[] he=0 & a=0 & pc=5 & k<N -> 1: (pc'=1) & (k'=k+1);
	[] ((he=0 & a=1) | (he=1 & a=0)) & cte>0 & pc=5 & k<N -> 1: (cte'=cte-1) & (he'=1) & (pc'=1) & (k'=k+1);
	[] ((he=0 & a=2) | (he=2 & a=0)) & cte<2 & pc=5 & k<N -> 1: (cte'=cte+1) & (he'=2) & (pc'=1) & (k'=k+1);
	[] ((he=1 & a=2) | (he=2 & a=1)) & pc=5 & k<N -> 1: (he'=0) & (pc'=1) & (k'=k+1);

endmodule
\end{lstlisting}

\begin{lstlisting}[language={Prism},
breaklines=true, breakatwhitespace=true, firstnumber=36, firstline=1, 
caption={TaxiNet system (with higher accuracy DNN).},
label={prism_full_high}]
    ...
    // M2 = Sensor || Perception (Higher Accuracy)
	[] cte=1 & pc=1 -> 0.962: (cte_est'=1) & (pc'=2) + 0.002: (cte_est'=0) & (pc'=2) + 0.036: (cte_est'=2) & (pc'=2);
	[] cte=0  & pc=1 -> 0.1: (cte_est'=1) & (pc'=2) + 0.9: (cte_est'=0) & (pc'=2);
    [] cte=2 & pc=1 -> 0.1: (cte_est'=1) & (pc'=2) + 0.9: (cte_est'=2) & (pc'=2);

	[] he=0 & pc=2 -> 0.9: (he_est'=0) & (pc'=3) + 0.05: (he_est'=1) & (pc'=3) + 0.05: (he_est'=2) & (pc'=3);	
	[] he=1 & pc=2 -> 0.1: (he_est'=0) & (pc'=3) + 0.9: (he_est'=1) & (pc'=3);
	[] he=2 & pc=2 -> 0.05: (he_est'=0) & (pc'=3) + 0.05: (he_est'=1) & (pc'=3) + 0.9: (he_est'=2) & (pc'=3);
    ...
 \end{lstlisting}




 

==> section_algorithm_bkp.tex <==
\section{Compositional Verification of an Autonomous System}

We illustrate our compositional approach via an example of an autonomous system, namely, an autonomous system for guiding airplanes on taxiways, as illustrated in Figure~\ref{fig:auto_system}.

The system consists of a {\em Perception} component, a {\em Controller}, the {\em Dynamics}, modeling the movement of an airplane on the taxiway, and the {\em Sensors}, e.g., camera, which may be subject to arbitrary perturbations from the environment in which the autonomous system operates.
%\ravi{Should we just call the Environment as Sensors? We are already using environment in a different sense when discussing about weakest assumptions.}\corina{I agree. I changed}
%
The controller sends commands $a$ to the dynamics, e.g., to  manoeuvre the airplane on the taxiway. The dynamics maps previous state $s$ and command $a$ to the next state $s'$. Some other information, such as velocity, may be provided as feedback to the controller but we ignore here for simplicity. The updated state $s'$ is read through sensors, such as cameras that generate high-dimensional images.
%Information about the environment is provided by the perception network , which  takes  high-dimensional images captured with a sensor (camera)  and returns its estimation $s_{est}$ of the real state $s$.
The perception network takes these high-dimensional images and returns its estimation $s_{est}$ of the actual state $s$.

There may be other sensors (radar, LIDAR, GPS) that we abstract away for simplicity.
Although very simple, this system resembles (semi)autonomous mechanisms that are already deployed in practice, such as adaptive cruise controllers and lane-keeping assist systems, which similarly use a DNN for visual perception to provide guidance to the software controlling electrical and mechanical subsystems of modern vehicles.


Suppose we want to check that the overall system satisfies a {\em safety property} $P$. For our example, one such safety property is that the airplane does not go off the runway, which can be expressed in terms of physical dimensions of the runway (see Section~\ref{sec:taxinet}).

In order to check this property, one can run many simulations, using,  e.g. XPlane~\cite{xplane} for our example.
However, simulation alone may not be enough to achieve the high degree of confidence in the  correctness of the system, necessary for deployment in a safety-critical setting (e.g., an airplane in our case).

We can write the system as the composition $\mathit{System}=\mathit{Sensors}\parop\mathit{Perception}\parop\mathit{Controller}\parop\mathit{Dynamics}$. Our goal is to formally verify $\mathit{System}\models P$. 
 
To do so we build a discrete model of the (airplane) dynamics and  a discrete-time controller for the system, similar to previous related work \cite{HoffmannTMT07,479140} which also considers discretized control.  
Treatment of more complex systems with continuous semantics is left for future work.
%\ravi{Perhaps we can also describe how to verify the system using assumptions here. Then, we can point out that either verification or constructing such assumptions with DNN in the loop is infeasible. I can try to write this.}\corina{yes please}
%

Directly using the weakest assumption generation algorithm described in Section~\ref{sec:assume_gen} on $\mathit{System}$ is infeasible due to the high complexity of the $\mathit{Perception}$ neural network (which may have thousands or millions of parameters) and the difficulty (or even impossibility) of precisely modeling the complex (high-definition) camera used to capture the images (i.e., the $\mathit{Sensor}$ component) that is subject to random environmental changes (e.g., changing weather and light conditions)
The main challenge that we address in the paper is the modeling of the $\mathit{Perception}$ (DNN) and $\mathit{Sensor}$ components in a manner that enables assumption generation.

%This is difficult due to high the complexity of the neural network(which may have thousands or millions of parameters), the complexity of the (high-definition) camera that is used to capture the images and the unpredictable nature of the environment, which is subject to random changes (e.g., changing weather and light conditions) which are difficult, if not impossible, to model precisely. 

\subsection{Abstractions For Perception}

To overcome these challenges, we propose to replace the perception component, 
%together with the environment and the sensor, 
together with the sensor, 
using simple abstractions that map the actuals to estimates for the system's states. 
Our analysis is performed in two steps, corresponding to two 'views' of the perception component -- {\em optimistic} and {\em pessimistic}. 

\begin{enumerate}
\item In the first step (optimistic view), we assume the perception is `perfect' and the abstraction maps each system state to the correct estimated state; thus we assume the DNN makes no mistake due to errors in training and/or unexpected perturbations in the environment. We can then check $\mathit{Perception}_{best}\parop\mathit{Controller}\parop\mathit{Dynamics}\models P$ using a formal verification tool (such as LTSA).
%
Even though this is an {\em idealized} scenario, the analysis is useful in practice as it allows to uncover and fix errors in the system that are due to possible wrong behaviour and interactions in the controller and dynamics, independent of any errors in perception.
%
After the above errors have been fixed we move on to the second step of the analysis. 

\item In the pessimistic view, we assume the {\em worst} about the DNN perception and use a non-deterministic abstraction $\mathit{Perception}_{worst}$ that relates every actual $s$ to every possible estimate $s_{est}$. This abstraction is conservative, as it accounts for any possible misprediction of the DNN, which may be due to poor training of the DNN, camera failures or unexpected conditions in the environment.
%, i.e., 
%$L(\mathit{Sensors}\parop \mathit{Perception})\subseteq L(\mathit{Perception}_{worst})$

The abstraction is built in the absence of any knowledge about the DNN, the camera, or the environment, and can thus enable analysis even {\em before} a DNN was trained. Furthermore the size of this non-deterministic abstraction is only proportional to the size of estimate vector\ravi{Should we say size of the set of possible DNN outcomes?}, and does not depend on the complexity of a particular DNN, of the high-definition camera or of the complex (or adversarial) environment conditions.

%TODO: to formalize as an LTS?

Once we have this abstraction, we can build a system $M=\mathit{Perception}_{worst}\parop\mathit{Controller}\parop\mathit{Dynamics}$ and check $M\models P$ using a formal verification tool (such as LTSA). 
%Note that due to the use of our conservative abstraction, $M$ is an abstraction of $\mathit{System}$, i.e. $L(\mathit{System})\subseteq L(M)$. 
However, this check is likely to fail, due to the over-approximation introduced by the non-deterministic abstraction, which may introduce many spurious behaviours in the system. To address this problem we extract a weakest assumption $A_{w,\Sigma}$ for $M$ that ensures that the safety property $P$ is satisfied; see Figure~\ref{fig:comp_verif}, where the conservative abstraction denotes $\mathit{Perception}_{worst}$.
\end{enumerate}

We can use this assumption to guide the development of a perception DNN and also as a basis of a safety monitor that ensures that the autonomous system satisfies the required property, as illustrated in Figure~\ref{fig:run-time}. The monitor checks the sequences of DNN outputs for conformance with the assumption, and traps those sequences that do not conform with it, as they will lead to a safety violation in the system.

\ravi{Made a pass till here}


\begin{figure}[t]
\centering
  \centering
  \includegraphics[width=0.8\linewidth]{AutonomousSystem.png}
  \captionof{figure}{Autonomous System using a DNN for Perception}
  \label{fig:auto_system}
\end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.7\linewidth]{CompVerif.png}
  \captionof{figure}{Compositional Verification}
  \label{fig:comp_verif}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{RunTime.png}
  \captionof{figure}{Autonomous System with Run-time Monitor}
  \label{fig:run-time}
\end{minipage}
\end{figure*}


\subsection{Automatically Generated Assumption}

In the case that $M\not\models P$, we leverage the weakest assumption  for $M$ with respect to property $P$.
This assumption can be built using the algorithm from ~\cite{ASE02}, which we summarized in Section~\ref{sec:background_assumption}.

For the autonomous system, the interface alphabet consists of the updates to the actual and estimated system state variables; let us denote it as $\Sigma_I= \mathit{Act} \cup \mathit{Est}$.

By construction, $A_{w,\Sigma_I}$ captures precisely the traces over  $\Sigma_I^*$ that ensure that the overall system does not violate the prescribed safety property, i.e. $A_{w,\Sigma_I}\parop M\models P$ (\divya{Is conjunction operator not applicable here, instead of parop operator?}). Furthermore, $A_{w,\Sigma_I}$ is the weakest, ensuring that  $A_{w,\Sigma_I}$ does not restrict $M$ unnecessarily.

We envision multiple uses for the assumption. For instance, it can be used for testing a candidate DNN to ensure that it follows the behaviour prescribed by the assumption. For our Taxiing application (see section~\ref{sec:taxinet}), the perception DNN is trained and tested based on images obtained from simulations, which naturally come in a sequence and therefore can be easily checked against the assumption. The assumption can also be used during the training of the DNN, in a neuro-symbolic way~\cite{}, as a specification of desired output for unlabelled real data, thus reducing the burden of manually labeling the input images. WE leave the exploration of these directions for future work.

The generated assumptions can be used as monitors deployed at run-time to ensure that the autonomous system guarantees the desired safety properties. One difficulty is that $\Sigma_I$ refers to labels in $Act$ which represent the actual values of the real system states.  As discussed, the autonomous system may not have access to the actual system state, and this is the very reason it uses a DNN, to get the estimated values of the system state (which we denoted by  $\mathit{Est}$).

While in some cases, it may be possible to  get the actual values through alternative means, e.g., through other sensors,  one can also set the alphabet of the assumption to be only in terms of the estimates received from the neural network, i.e., $\Sigma=Est$, and build the run-time monitor based on $A_{w,\Sigma}$. 

%By construction the assumption $A_w$ satisfies:
%$A_w \parop M\models P$

The following theorem states that the assumption indeed ensures that the autonomous system satisfies the required property. 

\begin{theorem}
If
%$Environment || Perception \models A_w$,
%(not sure about this bit)
$A_{w,\Sigma} \parop M\models P$, then
$ A_{w,\Sigma} || \mathit{System} \models P$.
\end{theorem}

This is true because $L(\mathit{System})\subseteq L(M)$, due to the nondeterministic abstraction. It follows $L(A_{w,\Sigma}\parop\mathit{System})\subseteq L(A_{w,\Sigma}\parop M)$. Since $L((A_{w,\Sigma}\parop M)\projop{\alpha P})\subseteq L(P)$, it follows that $L((A_{w,\Sigma}\parop \mathit{System})\projop{\alpha P})\subseteq L(P)$, i.e., $ A_{w,\Sigma} || \mathit{System} \models P$.

%$\mathit{Perception}_{worst}$ is an abstraction of $(\mathit{Perception} \parop \mathit{Sensors})\projop{\Sigma}$, for any $\mathit{Perception}$ and $\mathit{Sensors}$ components; i.e.,$L((\mathit{Perception} \parop \mathit{Sensors})\projop{\Sigma})\subseteq L(\mathit{Perception}_{worst})$.
%It follows that $L((\mathit{Perception} \parop \mathit{Sensors})\projop{\Sigma} \parop Controller \parop Dynamics)\subseteq L(\mathit{Perception}_{worst}\parop Controller \parop Dynamics)$.
%Also, $L((\mathit{Perception} \parop \mathit{Sensors})\projop{\Sigma} \parop Controller \parop Dynamics)\subseteq L(\mathit{Perception} \parop \mathit{Sensors} \parop Controller \parop Dynamics)$.
%... to formalize


%\subsection{Run-time Monitor}
%\todo{Other uses of assumption: testing the DNN over sequences, training the DNN etc.}

Since $A_{w,\Sigma}$ is modeled only in terms of the $Est$ alphabet, it follows that it can be deployed as a run-time monitor on the outputs of a neural network that is used by the autonomous system. Furthermore, from the theorem above, the monitor guarantees safety of the overall system. A good run-time monitor should not restrict a system unnecessarily; for instance, a monitor that blocks all the possible actions of a system may ensure safety but has no practical utility. Be construction, the assumptions that we use are guaranteed to be the weakest (i.e., most permissive) making them good candidates for run-time monitors.

We note the following property which relates weakest assumptions for different interface alphabets.

\begin{proposition}\label{prop}
Assume LTSs $M$, property $P$, and interface alphabet $\Sigma_I\subseteq \alpha M$. Assume also $\Sigma$, $\Sigma$ such that $\Sigma \subseteq \Sigma' \subseteq \Sigma_I$. Then, $L(A_{w,\Sigma})\subseteq L(A_{w,\Sigma'}) \subseteq L(A_{w,\Sigma_I})$.
\end{proposition}

%\corina{to prove?}
The intuition is that projection with a  smaller alphabet results in more behaviours in $M$ leading also to more error behaviours; consequently, the corresponding assumptions are more restrictive (contain less behaviours). Conversely, by adding actions to the interface alphabet, the corresponding assumption becomes weaker, more permissive. 

Thus, $A_{w,\Sigma}$ is only weakest with respect to a particular interface alphabet $\Sigma$. In section~\ref{sec:eval} we will describe an experiment that aims to quantify how permissive the assumption is for a realistic DNN that was trained for perception.

%We need the property of being "weakest" in justifying that this is a good runtime monitor since it does not restrict the system unnecessarily. Actually this assumption is only weakest with respect to the alphabet. See Proposition~\ref{prop}.

%\corina{note that if the algorithm for building the assumption returns false with the restricted alphabet, it means that we can not control the system only through monitoring the DNN actions; "false" may be spurious;  how to address: define monitor per initial state}


%Justify the use of Prism to quantify how {\em permissive} is the assumption in practice.

%$A_{w,\Sigma}$ can also be used for other activities ...
